Effective Targeted Attacks for Adversarial Self-Supervised Learning

Recently, unsupervised adversarial training (AT) has been highlighted as a means of achieving robustness in models without any label information. Previous studies in unsupervised AT have mostly focused on implementing self-supervised learning (SSL) frameworks, which maximize the instance-wise classification loss to generate adversarial examples. However, we observe that simply maximizing the self-supervised training loss with an untargeted adversarial attack often results in generating ineffective adversaries that may not help improve the robustness of the trained model, especially for non-contrastive SSL frameworks without negative examples. To tackle this problem, we propose a novel positive mining for targeted adversarial attack to generate effective adversaries for adversarial SSL frameworks. Specifically, we introduce an algorithm that selects the most confusing yet similar target example for a given instance based on entropy and similarity, and subsequently perturbs the given instance towards the selected target. Our method demonstrates significant enhancements in robustness when applied to non-contrastive SSL frameworks, and less but consistent robustness improvements with contrastive SSL frameworks, on the benchmark datasets.

==> Figure/Captions/class_analyze.tex <==
\begin{wrapfigure}[9]{r}{0.41\textwidth}
\vspace{-0.13in}
  \begin{center}
    \includegraphics[width=0.33\textwidth]{Figure/class_analyze.png}
  \end{center}
  \vspace{-0.1in}
  \caption{\small Percentage of predicted class}
  \label{figure:prediction_class}
\end{wrapfigure}

==> Figure/Captions/fig_tsne.tex <==
\begin{wrapfigure}[9]{r}{0.45\linewidth}
\vspace{-0.14in}
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/untarget.png}
        \caption{Untargeted attack}
        \label{fig:untarget_vis}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/target.png}
        \caption{Targeted attack}
        \label{fig:target_vis}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Visualize embedding}
    \label{figure:visualize}
\end{wrapfigure}

==> Figure/Captions/figure2.tex <==
\begin{figure*}
\centering{
\includegraphics[width=0.9\linewidth]{Figure/concept_fig.pdf}
}
\vspace{-0.2in}
\caption{\textbf{Overview of TAROSS on SimSiam.} Our approach consists of three parts: target selection, targeted attack, and adversarial self-supervised learning (SSL). We propose a simple and effective similarity- and entropy-based target selection that selects the maximum scored target based on score function ($\mathcal{S}$) (left). When we select the target image ($x_k$) for base instance ($x_i$), we conduct a targeted attack, which maximizes the similarity (middle). Then, we train the model with targeted adversarial examples (right).}
\label{fig:model_overview}
\vspace{-0.17in}
\end{figure*}


==> Figure/Captions/figure3.tex <==
\begin{wrapfigure}[17]{r}{0.3\textwidth}
\vspace{-0.3in}
    \centering{
    \includegraphics[width=\linewidth]{Figure/observation_3.png}
    }
    \caption{\textbf{Influence score based on similarity between source image and target image}}
    \label{fig:observe_1}
\end{wrapfigure}


==> Figure/Captions/figure4.tex <==
\begin{wrapfigure}[10]{r}{0.55\textwidth}
    \vspace{-0.15in}
    \begin{subfigure}{0.27\textwidth}
    \centering{
    \includegraphics[width=0.8\linewidth]{Figure/analyze2.png}
    }
    \captionof{figure}{Obfuscated gradient}
    \label{fig:analyze_2}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.27\textwidth}
    \centering{
    \includegraphics[width=0.8\linewidth]{Figure/analyze1.png}
    }
    \captionof{figure}{Training dynamic}
    \label{fig:analyze_1}
    \end{subfigure}
\end{wrapfigure}


==> Figure/Captions/figure5.tex <==
\begin{wrapfigure}[9]{r}{0.41\textwidth}
\vspace{-0.3in}
  \begin{center}
    \includegraphics[width=0.38\textwidth]{Figure/k_mean_clustering.png}
  \end{center}
  \vspace{-0.2in}
  \caption{\small K-means clustering target selection}
  \label{figure:kmeans}
\end{wrapfigure}

==> Figure/Captions/similarity_table.tex <==
\begin{figure}[t]
    \centering{
    \includegraphics[width=0.7\linewidth]{Figure/region_exp.pdf}
    }
\vspace{-0.1in}
\caption{\small Robustness of the model that conduct targeted attack based on similarity score which selecting the target image that are in pre-defined range ($r1,\cdots,r6$).}
\vspace{-0.2in}
\label{fig:observe_2}
\end{figure}


==> Figure/Captions/wrap_figure.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/untarget.png}
        \caption{Untargeted attack}
        \label{fig:untarget_vis}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/target.png}
        \caption{Targeted attack}
        \label{fig:target_vis}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Visualize embedding}
    \label{figure:visualize}
\end{figure}


==> Table/algorithm.tex <==
\setlength{\textfloatsep}{2pt}
\begin{algorithm}[t]
\caption{Targeted Attack Robust Self-Supervised Learning (TARO) for positive-pair-only SSL}
\begin{algorithmic}
\STATE {\bfseries Input:} Dataset $\mathcal{D}$, transformation function $\mathbf{t}$, model $f$, parameter of model $\theta$, target score function $\mathcal{S}$
\FOR{\texttt{iter} $\in$ number of iteration}
    \FOR{$x_i \in$ miniBatch $B=\{x_1, \dots, x_m\}$}
        \FOR{\texttt{n} in 2}
            \STATE Transform input $\mathbf{t}_n(x_i)$
            \STATE Find target images $\mathbf{t}_n(x_k)$ from $\mathcal{S}(\mathbf{t}_n(x_i), \mathrm{batch})$
            \STATE Generate targeted adversarial examples 
            \STATE \small $\delta^{t+1} = \Pi_{B(0,\epsilon)} \Big(\delta^t $
            \STATE \quad \small $+ \alpha \texttt{sign}\Big(\nabla_{\delta^t} \mathcal{L}_{\texttt{attack}}\big(\mathbf{t}_n(x_i)+\delta^{t}, \mathbf{t}_n(x_k)\big)\Big)\Big)$
            \STATE $\mathbf{t}_n(x_i)^{adv} = \mathbf{t}_n(x_i) + \delta^{t}$ 
        \ENDFOR
    \STATE Calculate training loss
    \STATE $\Lagr_{\texttt{TARO}} = \Lagr_{\texttt{selfsup}}(\mathbf{t}_1(x_i), \mathbf{t}_1(x_i)^{adv})$ 
    \STATE \quad \quad $+ \Lagr_{\texttt{selfsup}}(\mathbf{t}_1(x_i)^{adv}, \mathbf{t}_2(x_i)^{adv})$
    \STATE \quad \quad $+ \Lagr_{\texttt{selfsup}}(\mathbf{t}_2(x_i)^{adv}, \mathbf{t}_1(x_i))$
    \ENDFOR
% \STATE Optimize the weight $\theta$ over $\Lagr_{\texttt{TAROSS}}$ 
\STATE $\theta \leftarrow \theta - \beta\nabla_{\theta}\Lagr_{\mathtt{TAROSS}}$
\ENDFOR
\end{algorithmic}
\label{algo:algorithm}
\end{algorithm}


==> Table/multiple_benchmark_cifar100.tex <==
\begin{wraptable}{r}{0.5\linewidth}
\vspace{-0.1in}
\centering
\caption{Results of linear evaluation in a larger dataset, CIFAR-100. Rob. stands for robust accuracy against $\ell_{\infty}$ PGD attack.}
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{clcc}
\toprule
Attack loss & Method & Clean & Rob. \\
\midrule
Contrastive & RoCL & 45.99 & 17.17 \\
Contrastive & RoCL+TAROSS & \textbf{46.54} & \textbf{18.91} \\
\midrule
Positive-only & untargeted & 24.43 & 13.34 \\
Positive-only & TAROSS & \textbf{36.02} & \textbf{22.18} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{table:diff_dataset}
\vspace{-0.12in}
\end{wraptable}


==> Table/score_function_ablation.tex <==
\begin{figure}[t]
\begin{minipage}[t]{0.45\linewidth}
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/untarget.png}
        \caption{Untargeted attack}
        \label{fig:untarget_vis}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/target.png}
        \caption{Targeted attack}
        \label{fig:target_vis}
    \end{subfigure}
    \vspace{-0.1in}
    \caption{Visualize embedding}
    \label{figure:visualize}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\linewidth}
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/prob_target.pdf}
        \caption{Mean predict probability of base images}
        \label{fig:mean_softmax}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figure/num_target.pdf}
        \caption{Distribution of class of targeted images}
        \label{fig:targetclass_dist}
    \end{subfigure}
    \caption{Analysis of target from score function ($\mathcal{S}$)}
    \label{fig:analysis_target}
\end{minipage}
\end{figure}

==> Table/supple_table3.tex <==
\begin{table}[t]
\caption{\small Experimental results with white box attacks on ResNet18 trained on the CIFAR-100. Clean is the accuracy of clean images. All models are trained with $\ell_{\infty}$; thus the $\ell_{\infty}$ is the \emph{seen} adversarial attack.}
\centering
  \begin{tabular}{lcccc} %
    \toprule
    Method& Clean & AA &PGD $\ell_{\infty}$\\
    \midrule
    \multicolumn{3}{l}{\small{Self-supervised linear evaluation}}
    \\
    RoCL~\cite{kim2020rocl}\\
    ACL~\cite{jiang2020ACL}\\
    \textbf{Ours}\\
    \midrule
    \multicolumn{3}{l}{\small{Self-supervised robust linear evaluation}}
    \\
    RoCL~\cite{kim2020rocl}\\
    ACL~\cite{jiang2020ACL}\\
    Ours &\\
    \bottomrule
  \end{tabular}
\end{table}


==> Table/table0_blackbox.tex <==
\begin{table}[t]
\caption{Experimental results against black box PGD $\ell_{\infty}$ attacks on ResNet18 where all models are trained on the CIFAR-10.}
  \vspace{0.02in}
\centering
\begin{adjustbox}{width=\linewidth}
\label{table:blackbox_table0}
  \begin{tabular}{cclcccc} %
    \toprule
    \multicolumn{2}{c}{Self-supervised framework}&Method& Black box $\ell_{\infty}$\\
    \midrule
     \multirow{2}{*}{Contrastive}&SimCLR&RoCL~\cite{kim2020rocl}&59.73\\
      {}&SimCLR&ACL~\cite{jiang2020ACL}&\\
     \midrule
     Positive-only&SimSiam&Untargeted attack&\\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}

==> Table/table3.tex <==
\begin{table}[t]
\caption{\small Experimental results with white-box attacks on ResNet18 trained on CIFAR-10. Clean is the accuracy of clean images. All models are trained with $\ell_{\infty}$; thus, $\ell_{\infty}$ is the \emph{seen} adversarial attack.}
\centering
  \begin{tabular}{lcccccc} %
    \toprule
    &\multicolumn{3}{c}{ACL}&\multicolumn{3}{c}{Ours}\\
    \cmidrule(r){2-4}\cmidrule(r){5-7}
    Method & Clean & PGD $\ell_{\infty}$ & AutoAttack&Clean& PGD $\ell_{\infty}$ & AutoAttack\\
    \midrule
    Linear robust evaluation & \\
    Robust partial fine-tuning & \\
    Robust full fine-tuning & \\
    Robust gradual fine-tuning& \\
    \bottomrule
  \end{tabular}
  \label{table:table5}
\end{table}

==> Table/transfer_learning.tex <==
\begin{table}
\centering
\vspace{-0.13in}
    \caption{Results of adversarial transfer learning to CIFAR10 and CIFAR100.}
    \vspace{-0.05in}
    \begin{tabular}{lcccc}
        \toprule
        & \multicolumn{2}{c}{CIFAR10 $\rightarrow$ CIFAR100}& \multicolumn{2}{c}{CIFAR100 $\rightarrow$ CIFAR10}\\
        Method & Clean & PGD $\ell_{\infty}$ & Clean & PGD $\ell_{\infty}$\\
        \midrule
        RoCL~\cite{kim2020rocl} \\ 
        ACL~\cite{jiang2020ACL} \\
        Ours\\
        \bottomrule
    \end{tabular}
    \label{table:transfer_learning}
    \vspace{-0.4in}
\end{table}


==> Table/wrap_table.tex <==
\begin{table}[t]
\centering
    \caption{\small Results of our TAROSS with K-means clustering based-, and similarity based- selection for targeted attack on CIFAR5.}
    \begin{tabular}{ccc}
        \toprule
        {\small Selection}& Clean & PGD $\ell_{\infty}$\\
        \midrule
        {\small Untargeted*}&66.36&36.53\\
        {\small Random} &77.08&47.58\\
        {\small Similarity} & 76.04&48.73\\
        {\small K-means clustering} &  75.86&49.39\\
        \bottomrule
    \end{tabular}
    \vspace{-0.3in}
    \label{table:k_meanwrap_table}
\end{table}

